Rethinking Streaming Machine Learning Evaluation

While most work on evaluating machine learning (ML) models focuses on computing accuracy on batches of data, tracking accuracy alone in a streaming setting (i.e., unbounded, timestamp-ordered datasets) fails to appropriately identify when models are performing unexpectedly. In this position paper, we discuss how the nature of streaming ML problems introduces new real-world challenges (e.g., delayed arrival of labels) and recommend additional metrics to assess streaming ML performance.

==> researchdir.tex <==
In this section, we list a few interesting research ideas in streaming ML evaluation. 
% \agp{We only seem to dwell on delay. What about imbalance, window size}

\topic{Practically Handling Label Delays} Many applications of continual learning describe models that are fine-tuned immediately following each data example prior to the next prediction --- an approach that unrealistically assumes that manual labels can be collected instantaneously in response to label requests.
Work on progressive validation only starts to address this issue~\cite{blum_beating_1999, grzenda_delayed_2020}. In real-world settings, data points are usually sent to be labeled periodically in "batch" mode. If we impose a labeling budget and a constraint that labels can only be periodically obtained, how do state-of-the-art continual learning algorithms perform?

\topic{Benchmarks on Live Data Streams} Current streaming ML benchmarks involve a test set with a \emph{finite} number of data points. It would be interesting to have a benchmark that corresponds to a live data stream --- e.g., climate forecasting, real-time Wikipedia topic modeling, Ethereum gas price prediction. Because the task never ends and models may enter the competition at different times, comparing models in this setting may involve some recency bias encoded in the evaluation metric, possibly motivating different metrics than "cumulative accuracy."

\topic{Converting Static Distribution Shift Benchmarks to Continual Learning Benchmarks} Many of the distribution shift benchmarks involve a training set from distribution $D$ and test set from distribution $D'$, where $D \ne D'$. Most real-world distribution shifts happen gradually, not a single jump from one mode to another. How do we turn these datasets to gradually-changing? How do existing continual learning methods perform on such alterations of the benchmark?

% DROP

% There is a lot of work in active learning (i.e., selectively querying for labels on predictions made post-deployment) ...
